Materials Generation in the Era of Artificial Intelligence: A Comprehensive Survey

Materials are the foundation of modern society, underpinning advancements in energy, electronics, healthcare, transportation, and infrastructure. The ability to discover and design new materials with tailored properties is critical to solving some of the most pressing global challenges. In recent years, the growing availability of high-quality materials data combined with rapid advances in Artificial Intelligence (AI) has opened new opportunities for accelerating materials discovery. Data-driven generative models provide a powerful tool for materials design by directly create novel materials that satisfy predefined property requirements. Despite the proliferation of related work, there remains a notable lack of up-to-date and systematic surveys in this area. To fill this gap, this paper provides a comprehensive overview of recent progress in AI-driven materials generation. We first organize various types of materials and illustrate multiple representations of crystalline materials. We then provide a detailed summary and taxonomy of current AI-driven materials generation approaches. Furthermore, we discuss the common evaluation metrics and summarize open-source codes and benchmark datasets. Finally, we conclude with potential future directions and challenges in this fast-growing field. The related sources can be found at https://github.com/ZhixunLEE/Awesome-AI-for-Materials-Generation.

==> tables/meth.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|lllllllll}
\toprule
 & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Material}} & \multicolumn{2}{c}{\textbf{Task}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Code}} \\
 \cmidrule(lr){4-7} \cmidrule(lr){8-9}
                       &           &              & \textbf{IM}    & \textbf{MOF}    & \textbf{AS}   & \textbf{SC}   & \textbf{DCG}         & \textbf{CSP}        &   &    \\ \midrule
\multirow{12}{*}{\rotatebox{90}{\textbf{Diffusion}}}      & CDVAE \cite{xie2021crystal}      & SMLD                 & \true        & \false     & \false          & \false        \\
                                & DiffCSP \cite{jiao2023crystal}    & DDPM                 &          &      &           &         \\
                                & UniMat \cite{yang2023scalable}    & DDPM                 &          &      &           &         \\
                                & DiffCSP++ \cite{jiao2024space}  &                  &          &      &           &         \\
                                & GemsDiff \cite{klipfel2024vector}  &                  &          &      &           &         \\
                                & EquiCSP \cite{lin2024equivariant}  &                  &          &      &           &         \\
                                & FlowMM \cite{miller2024flowmm}     & RFM                 &          &      &           &         \\
                                & SuperDiff \cite{yuan2024diffusion}     &                  &          &      &           &         \\
                                & SymmCD \cite{levy2025symmcd}     &                  &          &      &           &         \\
                                & MOFDiff \cite{fu2023mofdiff}     & DDPM                 &          &      &           &         \\
                                & MatterGen \cite{zeni2025generative}     &                  &          &      &           &         \\
                                & MOFFlow \cite{kim2024mofflow}    & RFM                 &          &      &           &         \\
                                & CrystalFlow \cite{luo2024crystalflow}    & FM                 &          &      &           &         \\
                                & ADiT \cite{joshi2025all}    & LFM                 &          &      &           &         \\
                                & DAO \cite{wu2025siamese}    & DDPM                 &          &      &           &         \\ \midrule
\multirow{9}{*}{\rotatebox{90}{\textbf{Autoregressive}}} & G-SchNet \cite{gebauer2019symmetry}   &                  &          &      &           &         \\
                                & LM-CH/AC \cite{flam2023language}     &                  &          &      &           &         \\
                                & CrystaLLM \cite{antunes2024crystal}  & GPT-2          &  &  &       &          &      &           &   & \href{https://github.com/lantunes/CrystaLLM}{Link}       \\
                                & CrystalLLM \cite{gruver2024fine} & LLaMA-2                 &          &      &     &  &  &      &  & \href{https://github.com/facebookresearch/crystal-text-llm}{Link}        \\
                                & SLI2Cry \cite{xiao2023invertible}     &                  &          &      &           &         \\
                                & Mat2Seq \cite{yan2024invariant}    &                  &          &      &           &         \\
                                & MatExpert \cite{ding2024matexpert}    & LLaMA-2/3                 &          &      &   &  &  &        & 8B/70B & \href{https://github.com/BangLab-UdeM-Mila/MatExpert}{Link}       \\
                                & NatureLM \cite{xia2025naturelm}    &                  &          &      &           &         \\
                                & MatLLMSearch \cite{gan2025large}    &                  &          &      &           &         \\
                                & Uni-3DAR \cite{lu2025uni}    & -                 & \true         & \false     & \true    & \false & \true  & \true  & 90M & \href{https://github.com/dptech-corp/Uni-3DAR}{Link}        \\ \midrule
\multirow{4}{*}{\rotatebox{90}{\textbf{Hybird}}}         & FlowLLM \cite{sriram2024flowllm}    &                  &          &      &           &         \\
                                & GenMS \cite{yang2024generative}      &                  &          &      &           &         \\
                                & TGDMat \cite{das2025periodic}      &                  &          &      &           &         \\
                                & UniGenX \cite{zhang2025unigenx}      & NTP+DDPM                 &          &     &        &  &  &   & 100M/400M        \\ \midrule
\multirow{4}{*}{\rotatebox{90}{\textbf{Others}}}  & MatGAN \cite{dan2020generative}    & GAN                 &          &      &           &         \\       
& EMPNN \cite{klipfel2023equivariant}   & -           &  &  &      &          &    &          &      &   \href{https://github.com/aklipf/pegnn}{Link}  \\
& CubicGAN \cite{zhao2021high}   & GAN                 &          &      &           &         \\
                                & CrysBFN \cite{wu2025periodic}    & BFN                 &          &      &           &         \\ \bottomrule
\end{tabular}}
\end{table*}

==> tables/tree.tex <==

\definecolor{connect-line}{RGB}{0,0,0}
\definecolor{middle-color}{RGB}{255,255,255}

\definecolor{taxonomy-color}{RGB}{181, 168, 213}
\definecolor{material-color}{RGB}{181, 168, 213}
% \definecolor{material-color}{RGB}{154, 203, 208}

\definecolor{line-color}{RGB}{25,25,112}

\definecolor{black}{RGB}{0,0,0}

% \definecolor{pure}{RGB}{230,75,53}
% \definecolor{node}{RGB}{7,105,82}
% \definecolor{graph}{RGB}{207,134,0}

\definecolor{pure}{RGB}{38, 31, 179}
\definecolor{node}{RGB}{38, 31, 179}
% \definecolor{node}{RGB}{0, 106, 113}

\tikzstyle{pure-leaf}=[draw=pure,
    rounded corners,minimum height=1em,
    fill=taxonomy-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
]
\tikzstyle{pure-middle}=[draw=pure,
    rounded corners,minimum height=1em,
    fill=middle-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
]
    
\tikzstyle{node-leaf}=[draw=node,
    rounded corners,minimum height=1em,
    fill=material-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
]
\tikzstyle{node-middle}=[draw=node,
    rounded corners,minimum height=1em,
    fill=middle-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
]

\tikzstyle{leaf}=[draw=line-color,
    rounded corners,minimum height=1em,
    fill=leaf-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\tikzstyle{middle}=[draw=line-color,
    rounded corners,minimum height=1em,
    fill=middle-color!40,text opacity=1, align=center,
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]

    
\begin{figure*}[ht]
\centering
\begin{forest}
  for tree={
    forked edges,
    grow=east,
    reversed=true,
    anchor=base west,
    parent anchor=east,
    child anchor=west,
    base=middle,
    font=\scriptsize,
    rectangle,
    line width=0.9pt,
    draw=connect-line,
    rounded corners,align=left,
    minimum width=2em,
    s sep=5pt,
    inner xsep=3pt,
    inner ysep=1pt,
  },
  where level=1{text width=4.5em}{},
  where level=2{text width=6em,font=\scriptsize}{},
  where level=3{font=\scriptsize}{},
  where level=4{font=\scriptsize}{},
  where level=5{font=\scriptsize}{},
  [Material Generation with AI, black,rotate=90,anchor=north,edge=pure
    [Taxonomy, pure-middle, edge=pure, text width=4em
        [Diffusion-based, pure-middle, edge=pure, text width=7.8em
            [Score Matching with Langevin \\ Dynamics, pure-middle, text width=11.2em, edge=pure
                [CDVAE \cite{xie2021crystal}{,}  MOFDiff \cite{fu2023mofdiff}, pure-leaf, text width=21.7em, edge=pure]
            ]
            [Denoising Diffusion Probabilistic \\ Models, pure-middle, text width=11.2em, edge=pure
                [DiffCSP \cite{jiao2023crystal}{,} UniMat \cite{yang2023scalable}{,} \\ DiffCSP++ \cite{jiao2024space}{,} GemsDiff \cite{klipfel2024vector}{,} \\ EquiCSP \cite{lin2024equivariant}{,} SuperDiff \cite{yuan2024diffusion} \\ SymmCD \cite{levy2025symmcd}{,} MatterGen \cite{zeni2025generative}{,}\\ DAO \cite{wu2025siamese}{,}, pure-leaf, text width=21.7em, edge=pure]
            ]
            [Flow Matching, pure-middle, text width=11.2em, edge=pure
                [FlowMM \cite{miller2024flowmm}{,} MOFFlow \cite{kim2024mofflow}{,}\\CrystalFlow \cite{luo2024crystalflow}{,} ADiT \cite{joshi2025all}, pure-leaf, text width=21.7em, edge=pure]
            ]
        ]
        [Autoregressive-based, pure-middle, edge=pure, text width=7.8em
            [Crystallographic Information Files, pure-middle, text width=11.2em, edge=pure
                [CrystaLLM \cite{antunes2024crystal}{,} CrystalLLM \cite{gruver2024fine}{,}\\LM-CH/AC \cite{flam2023language}{,} MatExpert \cite{ding2024matexpert}{,}\\MatLLMSearch \cite{gan2025large}, pure-leaf, text width=21.7em, edge=pure]
            ]
            [Other Sequences, pure-middle, text width=11.2em, edge=pure
                [G-SchNet \cite{gebauer2019symmetry}{,} SLI2Cry \cite{xiao2023invertible}{,}\\Mat2Seq \cite{yan2024invariant}{,} Uni-3DAR \cite{lu2025uni}{,}\\NatureLM \cite{xia2025naturelm}{,} MatLLMSearch \cite{gan2025large}, pure-leaf, text width=21.7em, edge=pure]
            ]
        ]
        [Hybird Method, pure-middle, edge=pure, text width=7.8em
            [Diffusion + Autoregressive, pure-middle, text width=11.2em, edge=pure
                [FlowLLM \cite{sriram2024flowllm}{,} GenMS \cite{yang2024generative}{,}\\TGDMat \cite{das2025periodic}{,} UniGenX \cite{zhang2025unigenx}, pure-leaf, text width=21.7em, edge=pure]
            ]
        ]
        [Others, pure-middle, edge=pure, text width=7.8em
            [MatGAN, pure-leaf, text width=34.8em, edge=pure]
        ]
    ]
    [Materials, node-middle, edge=node, text width=4em
        [Inorganic Crystals, node-middle, edge=node,text width=7.8em
            [CDVAE \cite{xie2021crystal}{,} DiffCSP \cite{jiao2023crystal}{,} UniMat \cite{yang2023scalable}{,} DiffCSP++ \cite{jiao2024space}{,}\\GemsDiff \cite{klipfel2024vector}{,} EquiCSP \cite{lin2024equivariant}{,} FlowMM \cite{miller2024flowmm}{,}\\SymmCD \cite{levy2025symmcd}{,} MatterGen \cite{zeni2025generative}{,} CrystalFlow \cite{luo2024crystalflow}{,}\\ DAO \cite{wu2025siamese}{,} CrystalGRW \cite{tangsongcharoen2025crystalgrw}{,} CrystaLLM \cite{antunes2024crystal}{,}\\CrystalLLM \cite{gruver2024fine}{,} SLI2Cry \cite{xiao2023invertible}{,} Mat2Seq \cite{yan2024invariant}{,}\\MatExpert \cite{ding2024matexpert}{,} MatLLMSearch \cite{gan2025large}{,} FlowLLM \cite{sriram2024flowllm}{,}\\GenMS \cite{yang2024generative}{,} TGDMat \cite{das2025periodic}{,} MatGAN \cite{dan2020generative}{,}\\EMPNN \cite{klipfel2023equivariant}{,} CGWGAN \cite{su2024cgwgan}{,} CrysBFN \cite{wu2025periodic}, node-leaf, text width=34.8em, edge=node]
        ]
        [Atomic Systems, node-middle, edge=node, text width=7.8em
            [ADiT \cite{joshi2025all}{,} G-SchNet \cite{gebauer2019symmetry}{,} LM-CH/AC \cite{flam2023language}{,}\\NatureLM \cite{xia2025naturelm}{,} Uni-3DAR \cite{lu2025uni}{,} UniGenX \cite{zhang2025unigenx}, node-leaf, text width=34.8em, edge=node]
        ]
        [Others, node-middle, edge=node, text width=7.8em
            [Metal-organic Frameworks, pure-middle, text width=11.2em, edge=pure
                [MOFDiff \cite{fu2023mofdiff}{,} MOFFlow \cite{kim2024mofflow}, pure-leaf, text width=21.7em, edge=pure]
            ]
            [Organic Crystals, pure-middle, text width=11.2em, edge=pure
                [DeepCSP \cite{ye2024organic}, pure-leaf, text width=21.7em, edge=pure]
            ]
            [Superconductors, pure-middle, text width=11.2em, edge=pure
                [SuperDiff \cite{yuan2024diffusion}, pure-leaf, text width=21.7em, edge=pure]
            ]
        ]
    ]
  ]  
\end{forest}

\caption{A taxonomy of generative models for materials with representative works.}
\label{fig:taxonomy-techniques}
\end{figure*}
